Learning Frame-Wise Emotion Intensity for Audio-Driven Talking-Head Generation

Human emotional expression is inherently dynamic, complex, and fluid, characterized by smooth transitions in intensity throughout verbal communication. However, the modeling of such intensity fluctuations has been largely overlooked by previous audio-driven talking-head generation methods, which often results in static emotional outputs. In this paper, we explore how emotion intensity fluctuates during speech, proposing a method for capturing and generating these subtle shifts for talking-head generation. Specifically, we develop a talking-head framework that is capable of generating a variety of emotions with precise control over intensity levels. This is achieved by learning a continuous emotion latent space, where emotion types are encoded within latent orientations and emotion intensity is reflected in latent norms. In addition, to capture the dynamic intensity fluctuations, we adopt an audio-to-intensity predictor by considering the speaking tone that reflects the intensity. The training signals for this predictor are obtained through our emotion-agnostic intensity pseudo-labeling method without the need of frame-wise intensity labeling. Extensive experiments and analyses validate the effectiveness of our proposed method in accurately capturing and reproducing emotion intensity fluctuations in talking-head generation, thereby significantly enhancing the expressiveness and realism of the generated outputs.

==> abstract.tex <==
We convey our emotions through facial expressions and verbal communication in a dynamic and complex manner. The emotion can be more intense at certain key points in a sentence, and the way emotion intensity changes can even imply semantics, possibly indicating the direct subject we intend to address. However, the intensity of emotion and how we express it throughout our speech is still an underexplored area. This paper studies how emotion intensity fluctuates in talking head videos and contributes a talking head generator that can precisely mimic those using only the audio as input. To this end, we propose three key components: 1) a method to pseudo-label these intensity shifts from the video frames, 2) an audio-to-intensity mapping to infer intensities from the input audio, and 3) a video generator that can produce talking heads with accurate emotion and intensity.

More specifically, we propose to use key-point distances as proxies for emotion intensity, and we train a conditional VAE model to predict those intensities from audio. To generate video with per-frame accurate emotional intensity, we construct a latent space where different emotions and their intensity are naturally disentangled yet still linked together via the neutral emotion and their semantic relationships. This latent space allows our method to effectively capture subtle intensity shifts in data (which was challenging to do before) and accurately generate talking heads with varying intensity. Our experiments show that our method generates videos with more accurate emotion with respect to both the emotion type and the intensity. Various user studies further confirm the superiority of our method where our generated samples are consistently rated as more realistic, diverse, and natural.

==> backup.tex <==
\begin{table*}[!ht] 
\centering
\resizebox{0.95\textwidth}{!}{%
  \begin{tabular}{l|c|ccc|ccc}
    \toprule
   \multirow{2}{*}{Method} & {Emotion} & \multicolumn{3}{c|}{Video Quality} & \multicolumn{3}{c}{Lip Synchronization} \\
    & Acc & SSIM $\uparrow$ & PSNR $\uparrow$ & FID $\downarrow$ & SyncNet $\uparrow$ & M-LMD $\downarrow$ & F-LMD $\downarrow$ \\
    \midrule
   {ATVG \cite{XuCVPR}}  & 17.36
 & {0.56} & {17.64} & 99.42  & {1.80} & {2.77}  & 3.74  \\
   {Wav2Lip \cite{Ranjan2021LearningTC}}  & 
   17.87  & {0.57} & {19.12} & 67.49  & \textbf{8.97} & {3.11}  & 3.71  \\
     %BMNet \cite{Shi2022SimiCounting}  &  & 32.39 & 46.01 & 1.75 & 9.86 & 36.94 & 46.73 & 1.65 & 9.46 \\
     MakeItTalk  \cite{Shi2022SimiCounting}  & 15.23 & 0.55 & 18.79 & 51.88 & 5.28 & 3.61 & 4.00 \\
     AVCT  \cite{You2022FewshotOC}  & 15.64  & 0.54 & 18.43 & 39.18   & 6.02 & 3.82 & 4.33 \\
    {PC-AVS \cite{Ranjan2021LearningTC}}  & 11.88 & {0.61} & {20.60} & 53.04 & {8.60} & {2.66}  & 2.70  \\
    EAMM \cite{Ranjan2021LearningTC} & 49.85  &  {0.66} & {20.55} & {22.38}  & 6.62 & \textbf{2.19} & 2.55 \\
    EAT \cite{Shi2022SimiCounting} & 75.43 &  {0.68} & {21.75} & {19.69}  & 8.28 & 2.25 & 2.47 \\
    Ours & \textbf{83.55} & \textbf{0.83} & \textbf{23.66} & \textbf{16.77}  & {8.31} & {2.26} & \textbf{2.40} \\
    \midrule
    Ground-Truth & 84.37 &  {1.00} & $\infty$ & {0}  & 7.76 & 0.00 & 0.00 \\
    \bottomrule
  \end{tabular}
  } \\
 \caption{ Quantitative comparisons with state-of-the-art methods on MEAD \cite{}. 
  }\label{tab:mead_results} 
\end{table*}



\begin{table*}[!ht] 
\centering
\resizebox{0.84\textwidth}{!}{%
  \begin{tabular}{l|ccc|ccc}
    \toprule
   \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Video Quality} & \multicolumn{3}{c}{Lip Synchronization} \\
     & SSIM $\uparrow$ & PSNR $\uparrow$ & FID $\downarrow$ & SyncNet $\uparrow$ & M-LMD $\downarrow$ & F-LMD $\downarrow$ \\
    \midrule
   {ATVG \cite{Xu__CVPR}}  
 & {0.64} & {18.40} & 51.56  & {2.73} & {2.69}  & 3.31  \\
   {Wav2Lip \cite{Ranjan2021LearningTC}}  & 
   {0.73} & {22.80} & 7.44  & \textbf{7.59} & {1.58}  & 2.47  \\
     %BMNet \cite{Shi2022SimiCounting}  &  & 32.39 & 46.01 & 1.75 & 9.86 & 36.94 & 46.73 & 1.65 & 9.46 \\
     MakeItTalk  \cite{Shi2022SimiCounting}  & 0.69 & 21.67 & 3.37 & 3.28 & 2.16 & 2.99 \\
     AVCT  \cite{You2022FewshotOC}   & 0.68 & 21.72 & 2.01   & 4.63 & 2.55 & 3.23 \\
    {PC-AVS \cite{Ranjan2021LearningTC}}  & {0.72} & {23.32} & 4.64 & {7.36} & \textbf{1.54}  & 2.11  \\
    EAMM \cite{Ranjan2021LearningTC} &  {0.71} & {22.34} & {6.44}  & 4.67 & {1.81} & 2.37 \\
    EAT \cite{Shi2022SimiCounting} &   {0.77} & {24.11} & {3.52}  & 6.22 & 1.79 & 2.08 \\
    Ours &  \textbf{0.85} & \textbf{25.63} & \textbf{1.88}  & {6.20} & {1.70} & \textbf{1.75} \\
    \midrule
    Ground-Truth  &   {1.00} & {$\infty$} & {0}  & 7.06 & 0.00 & 0.00 \\
    \bottomrule
  \end{tabular}
  } \\
 \caption{ Quantitative comparisons with state-of-the-art methods on LRW \cite{}. 
  }\label{tab:lrw_results} 
\end{table*}

==> checklist.tex <==


\newpage
%\clearpage
\section{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, the main contributions have been clearly stated. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, in section \ref{sec:conclusion-limitation}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  We do not include theoretical results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All implementation details have been included and we will make the code available.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes. All codes and trained models will be made available.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes. All parameter settings are included in the implementation details.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: It is not the common practice to report the error bars due to the large datasets. Testing requires heavy computational resources.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: N/A
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No ethical issues significant enough that we feel need to be explicitly mentioned.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: N/A
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: N/A
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All codes and models are properly credited.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No new asset.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: N/A
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No risk involved.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> rebuttal_bkup.tex <==
<!---
Following Wav2Lip, given a talking-head video and the corresponding speech, we first compute the cosine similarity between the video embedding $v$ and the speech embedding $s$. This similarity indicates the probability that the input audio-video pair is in sync. We calculate $L_{sync}$ as the negative log-likelihood of this cosine similarity: $L_{sync} = -\textnormal{log} \frac{v \cdot s} {max(\lVert v \lVert \cdot \lVert s \lVert, \epsilon)}$, and minimize $L_{sync}$ during training. To extract $v$ and $s$, we follow Wav2Lip and utilize the image encoder and speech encoder from SyncNet.
-->

==> sec1_backup.tex <==
\section{Introduction}



Audio-driven talking-head synthesis \cite{das2020motion,EAT,sad-talker,pc-avs,wav2lip} has drawn increasing attention due to its wide range of applications in various fields such as virtual reality, digital humans \cite{Ad-nerf}, and assistive technologies. Recently, many works
have focused on synchronizing lip movements with speech content \cite{wav2lip, chen2018lip,chen2020rhythmic,song2018rnn}.
However, in addition to speech, humans also convey intentions through emotional expressions. Hence, developing emotionally expressive talking-heads is crucial to enhance the fidelity of these systems for real-world applications. 

Unlike static displays of emotion, our emotional expressions are inherently dynamic and fluid with smooth transition in terms of emotion intensity levels. Imagine a scenario where someone receives unexpected good news. Initially, they may smile slightly as they process it. As they fully comprehend, their smile might widen and their eyes might brighten, reflecting growing excitement and happiness. This progression illustrates the dynamic nature of human expressions with smooth shifts in emotion intensity levels, unlike static displays such as a fixed smile.

While there have been previous efforts to generate emotion-aware talking-heads \cite{EAT,SPACE,mm-esl,evp}, the natural fluctuations in intensity levels have been largely overlooked. Addressing this requires the model to 1) infer smooth emotion intensity flows based on audio cues and 2) precisely generate facial expressions that correspond to the inferred intensity levels.
%
However, capturing these intensity fluctuations can be challenging in existing emotional-aware talking-head methods: 1) the model would rely on frame-wise intensity annotations, which are difficult to obtain in practice; 2) there should be mechanisms to control the generated intensity precisely, instead of homogeneous outputs.
% However, capturing these intensity fluctuations requires frame-wise intensity annotations, which are unavailable in current datasets.
% %
% Moreover, we find that existing emotional-aware talking-head methods struggle to control the generated intensity precisely, often resulting in homogeneous outputs.


In this paper, we present a talking-head generation system that effectively captures emotion intensity fluctuations and precisely generates the corresponding facial expressions. To this end, our first step is to develop a talking-head generator capable of generating a variety of emotion categories with precise control over intensity levels. Specifically, we propose to learn a continuous emotion latent space in which emotion category is represented by the latent orientation and emotion intensity is represented by the latent norm. Notably, for neutral emotion, we consider the intensity to be zero and position it at the origin of the latent space. Our intuition is that the intensity level should positively correlate with the deviation from a neutral expression. Through our reorganization method, this deviation is intrinsically encoded in the distance from the origin point in the latent space, {i.e.}, latent norm. Consequently, latent features that correspond to the same intensity would lie on the same hypersphere, with norms representing intensity levels.

We use the embeddings in this emotion latent space as input conditions to guide a transformer-based model to generate emotional facial expressions.  Through both qualitative and quantitative analyses, we demonstrate the effectiveness of our proposed latent space reorganizing method in precise control over emotion category and intensity levels.

To further capture the emotion intensity fluctuations in speech, we introduce an emotion-agnostic intensity pseudo-labeling method. This method quantifies the emotion intensity of any given frame by measuring keypoint distances between the current frame and its corresponding neutral frame. These frame-wise pseudo intensities will then serve as regression targets for training an audio-to-intensity predictor. 
During inference, we leverage the trained audio-to-intensity predictor to infer audio-synchronized intensity fluctuations from the speaking tone, {i.e.}, audio inputs. These fluctuations are then transformed into intensity-aware emotion features within the proposed emotion latent space, guiding the generation of realistic talking-head videos with natural intensity flows.

Our main contributions can be summarized as follows:
\begin{itemize}
    \item We present a novel approach for reorganizing the latent space of emotions in talking-head generation, enabling both diverse emotional expressions and precise control over intensity levels.
    \item We propose an emotion-agnostic intensity pseudo-labeling method that accurately quantifies the intensity of any given frame based on keypoint distance.
    
    \item We introduce an audio-to-intensity predictor, which captures the dynamics of emotion intensity in response to changes in audio input. 
\end{itemize}

==> sec3_backup.tex <==
\section{Method}
\label{method}

In this section, we introduce our proposed method for generating talking-heads with frame-wise emotion intensity. 
%
Figure \ref{fig:pipeline} gives an overview of the pipeline, which involves intensity-aware emotion latent space reorganization, pseudo-labeling emotion intensity per frame, and training an intensity prediction model based on audio inputs. In the following subsections, we will first elaborate on these three components, and then describe the inference process of our method.

\subsection{Emotional Talking-Head Model Training}
\subsubsection{Emotion-Agnostic Pre-training}
We first pre-train an emotion-agnostic talking-head generation model following \cite{EAT}. This model comprises an audio-to-expression transformer and a talking-head generator. The transformer first produces 3D expression keypoints, which are then used by the generator to generate video frames. Although this model showcases impressive results in terms of lip synchronization and video quality, it lacks the capability for emotional expression generation or control over intensity levels. 


\subsubsection{Emotion Latent Space Reorganization}

To enable emotional talking-head generation, we propose to learn a continuous emotion latent space where the latent embeddings serve as guidance to steer the transformer in generating different emotional expressions. 
Specifically, we expect this latent space to 1) accommodate features of diverse emotion categories, and 2) encode corresponding intensity levels. Furthermore, we aim for disentanglement between the encoded emotion category and intensity, thereby allowing for flexible control over both.
To do this, we reorganize the latent space such that emotion category information is encoded in the latent orientation, while intensity information is encoded in the latent norm. For neutral emotion, we consider the intensity to be zero and position it at the origin of the latent space.

Since the current emotional dataset, {i.e.}, MEAD \cite{mead}, only contains training videos of the eight basic emotions, we leverage the robust generalizability of the pre-trained CLIP \cite{clip} space to enable the generation of more diverse emotions. Specifically, for an input video with emotion label $e$ and intensity label $i$, we extract the corresponding text embedding $f_e$ from the CLIP text encoder. An adaptation network $M$ is then adopted to map $f_e$ to our proposed emotion latent space. In the case where $e$ represents neutral emotion, we minimize the L2-norm of the emotion feature $M(f_e)$ to enforce it to center around the origin. Otherwise, for non-neutral emotions, we re-scale $M(f_e)$ to $M^r(f_e)$ such that $\|M^r(f_e)\| = t(e)$, where $t(e)$ is positively correlated with $e$. This ensures that the features of the same intensity will be mapped to the same hypersphere, with norms representing intensity levels. Meanwhile, the location on this hypersphere is determined by the emotion category.


\begin{figure}
\begin{center}
\hspace{-6mm}
\includegraphics[width=1.03\columnwidth]{figs/pipeline_talking.pdf} \vspace{1mm}
\caption{
An overview of our proposed method. 
%We propose to learn a continuous emotion latent space in which emotion categories are encoded within latent orientations, and emotion intensity is reflected in latent norms.
To generate talking-heads with fluid intensity transitions, we first infer these fluctuations from audio inputs using an audio-to-intensity predictor. The training targets for this predictor are obtained through our emotion-agnostic intensity pseudo-labeling method. 
Then, for a specified driving emotion (e.g., \textit{happy}), we map it onto our proposed emotion latent space and adjust its norm based on the inferred intensity fluctuations. These resulting intensity-aware emotion features then serve as guiding signals for a transformer-based talking-head generation model, enabling the generation of lifelike talking-head videos.
%These fluctuations are then transformed into intensity-aware emotion features within the proposed emotion latent space, guiding the transformer model to gene
%We use the same model configuration for images of top / bottom rows with the only difference being the initial noise. 
} \vspace{-2mm}
\label{fig:pipeline}
\end{center}
\end{figure}


\subsubsection{Training Objectives}
We input the re-scaled emotion features to the transformer as a guidance to generate emotional expressions. Specifically, this guidance is integrated as an additional input token of the transformer layer following \cite{EAT}. The final loss for training the talking-head model is calculated as follow:
\begin{equation}\label{eq:loss}
    L = \lambda_{exp} * L_{exp} + \lambda_{rec} * L_{rec} + \lambda_{sync} * L_{sync} + \lambda_{norm} * L_{norm},
\end{equation}
where $\lambda_{exp}$, $\lambda_{sync}$, $\lambda_{rec}$, $\lambda_{norm}$ are hyper-parameters that re-weight the corresponding loss term. $L_{exp}$ represents the mean square error between the ground-truth expression keypoints and the corresponding keypoints predicted by the transformer. 
$L_{rec}$ is the L1 reconstruction loss between the generated frame and the input frame within the facial region.
$L_{sync}$ is the lip synchronization loss introduced in Wav2Lip \cite{wav2lip}.
$L_{norm}$ denotes the L2-norm of the emotion feature, which only applies for neutral emotion.
%As shown in Figure \ref{fig:re-organization}, our reorganized latent space achieves improved separability between different emotional categories and offers flexible control over intensity levels.

%Specifically, we propose reorganizing this latent space to encode emotional type information in the latent orientation and intensity information in the latent norm, thereby facilitating disentanglement and flexible control over both aspects of emotional expression generation.
\subsection{Frame-Wise Intensity Pseudo-labeling}
While the mentioned model offers flexible control over emotion intensity levels for talking-head generation through latent norms, capturing the dynamic fluctuations in intensity during natural speech is crucial for realistic results.
To address this, we introduce an emotion-agnostic intensity pseudo-labeling method that quantifies the intensity level of any given frame.

Specifically, given a talking-head frame $i$ and the corresponding expression keypoints $K_i$, we extract the expression keypoints $K_i^N$ from the neutral face of the same person. 
The pseudo intensity $I_i$ is computed as the sum of absolute difference between $K_i$ and $K_i^N$. Essentially, a greater deviation between the given expression and the neutral facial expression indicates a higher intensity level, while a lower deviation suggests a lower intensity level.
%The expression 3D offset is then computed as the L1 distance between $K_i$ and $K_i^N$. This 3D offset quantifies how the given expression differs from the neutral facial expression.
%We then flatten the 3D expression offset to a 1D vector and take the sum over all dimensions. 

\subsection{Audio-to-Intensity Prediction}
To further estimate the pseudo intensity fluctuations from audio inputs during inference, we introduce a variational auto-encoder (VAE)-based model for audio-to-intensity prediction. This model predicts the pseudo-labeled emotion intensity conditioned on audio inputs, as the speaking tone often reflects the emotion intensity when people talk. To obtain audio representations, we utilize Hu-BERT \cite{hubert}, a state-of-the-art automatic speech recognition model to extract audio features $a$ from the input waveform. Throughout training, the intensity predictor ($P$) is trained to predict the entire sequence of pseudo intensity using an encoder-decoder structure. The training loss of this predictor can be written as follows:
\begin{equation}\label{eq:vae_loss}
    L_{P}(\phi, \theta, \epsilon) = -\textnormal{E}_{q_\phi(z|I,a)}[\textnormal{log}p_\theta(I|z, a)] + \textnormal{KL}(q_\phi(z|I,a)|p_\epsilon(z|a)),
\end{equation}
where $\phi, \theta, \epsilon$ denote the model parameters of the encoder, decoder and the VAE prior, respectively. A normalizing flow is employed to establish a time-related distribution as the prior, following the approach in \cite{GeneFace}.
We provide further details about the architecture of the encoder and decoder in the supplementary materials.

\subsection{Intensity-Aware Emotional Talking-head Generation}

Our goal is to generate talking-head videos with emotion intensity fluctuations that correspond to changes in audio inputs. In particular, given an input audio and a driving emotion, we first infer the emotion intensity $\hat{I}$ using our trained audio-to-intensity predictor. The predicted intensity $\hat{I}$ is represented as a sequence of scalars. 
To generate the talking-head videos, we map the CLIP embedding of the driving emotion to our proposed emotion latent space. This emotion embedding is then re-normalized according to the predicted intensity $\hat{I}$, resulting a sequence of embeddings with the same latent direction but varying latent norms. With this sequence of intensity-aware emotion embeddings, we can then leverage them to guide the transformer model in generating talking-head videos with frame-wise intensity fluctuations.

==> tmp.tex <==
\section*{Response to Reviewer EC1Z}
\textbf{r/c - s/p/contribution}

\textbf{5/4 - 3/3/2}

We thank the reviewer for the valuable feedback. We are very encouraged to see that the reviewer finds that our proposed method is simple and effective, with reliable results and thorough analysis. We address the major questions and concerns below.

\begin{quote}
To enhance reproducibility, the transformer model architecture needs more detailed explanations. What are the specific architectural details of the transformer model used in the talking-head generation? How does it integrate with the continuous emotion latent space?
\end{quote}

Thank you for the question. The transformer model used in our method consists of an encoder and a decoder. The encoder takes a sequence of audio tokens as input, each of which is a 128-dimensional vector. Both the encoder and decoder contain six transformer layers with eight attention heads. Each transformer layer includes a feed-forward network consisting of two fully connected (FC) layers, with the hidden dimension set to 1024. To integrate with the continuous emotion latent space, we incorporate the emotion latent feature as an additional input token into each layer of the transformer architecture. Additionally, following \cite{1}, we employ a lightweight sub-network that takes the emotion latent features as input to predict emotion-related keypoint deformations. These predicted keypoint deformations are then added to the output of the transformer to obtain the final expression keypoints. We will include these details and publish the code to enhance reproducibility.

\begin{quote}
The training loss for the audio-to-intensity predictor is distinct from the final training loss of the overall model. Could you elucidate whether the audio-to-intensity predictor is trained separately from the rest of the system? What are the advantages of this approach compared to an end-to-end training strategy?
\end{quote}

Thank you for the question. The audio-to-intensity predictor is indeed trained separately from the rest of the system. The talking-head generator is trained on MEAD, which is a high-quality emotion dataset captured in a strictly-controlled environment with carefully selected actors. While this dataset is beneficial for learning accurate facial expressions for various emotions, it lacks diversity and naturalness in audio. To address this, we train the audio-to-intensity predictor separately using Voxceleb2, a real-world dataset that provides a wide variety of audio inputs. However, the emotion expressions in Voxceleb2 may be noisy, which can affect the model's ability to learn accurate emotions. By training the two components separately on two datasets, we can effectively leverage the strengths of each: MEAD for its precise emotional expressions and Voxceleb2 for its diverse real-world audio inputs.

\begin{quote}
How does the proposed method perform with real-world audio inputs that may be diverse and noisy? Are there any preprocessing steps required to handle such inputs?
\end{quote}

Thank you for the question. 

\begin{quote}
What are the limitations of scaling this approach to more complex emotional landscapes or larger datasets? How do you plan to address these challenges in future work?
\end{quote}

\section*{Response to Reviewer 7AV4}
\textbf{r/c - s/p/contribution}

\textbf{7/3 - 3/3/3}

We thank the reviewer for the valuable feedback. We are very encouraged to see that the reviewer finds that our method has a well-elaborated framework with notable performance improvements and thorough analyses. We address the major questions and concerns below.

\begin{quote}
The design of the pseudo emotion space lacks justification or further analysis. Although the proposed framework is validated to improve generation results, the experiments only partially show the relations between the pseudo labels to the ground truth emotions.
\end{quote}

A:

\begin{quote}
The ambiguity of synchronization evaluation leads to biased evaluation.
\end{quote}

A: 

\begin{quote}
The authors should include case studies with continuous frames to demonstrate the effectiveness of continuous emotion-aware generation.
\end{quote}

\begin{quote}
Additional evaluation datasets would convince readers for the model effectiveness.
\end{quote}

Thank you for the suggestion. We evaluate our method on an additional test set, HDTF \cite{Zhang2021}, as suggested. We present the results in the table below. The performance improvements validate the effectiveness of our method. We will include these results.

\begin{table}[h]
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Method & SSIM $\uparrow$ & PSNR $\uparrow$ & FID $\downarrow$ & SyncNet $\uparrow$ & F-LMD $\downarrow$ \\
\hline
MakeItTalk & 0.55 & 18.68 & 25.42 & 4.76 & 4.05 \\
AVCT & 0.57 & 18.73 & 20.48 & 6.65 & 3.72 \\
PC-AVS & 0.72 & 20.74 & 23.57 & 7.68 & 2.89 \\
EAMM & 0.75 & 21.12 & 22.45 & 6.78 & 3.03 \\
EAT & 0.78 & 21.36 & 20.96 & 7.43 & 2.86 \\
Ours & \textbf{0.82} & \textbf{21.80} & \textbf{18.19} & \textbf{7.75} & \textbf{2.62} \\
\hline
\end{tabular}
\caption{Performance comparison on the HDTF dataset.}
\end{table}

\begin{quote}
Why the author choose an ASR-based model for audio features? Why not using wav2vec2 that has shown strong effectiveness to multiple emotion tasks?
\end{quote}

A:

\begin{quote}
What is the exact function of t in line 156? How will this function affect the generation results?
\end{quote}

A:

\section*{Response to Reviewer DU7K}
\textbf{r/c - s/p/contribution}

\textbf{6/4 - 3/3/3}

We thank the reviewer for the valuable feedback. We address the major questions and concerns below.

\begin{quote}
It is recommended to provide a detailed explanation of the notations in Equation (1), such as L and a.
\end{quote}

Thank you for the suggestion. In Eq. (1), L denotes the pseudo emotion intensity and $a$ denotes the audio input. We will clarify this carefully.

\begin{quote}
Regarding the novel emotion-agnostic intensity pseudo-labeling method in the paper (in Section 3.1), I suggest illustrating the idea with diagrams. For instance, the calculation of the pseudo intensity could be depicted through a comparative illustration of expression keypoints and neutral keypoints. This can then be explained in conjunction with the model diagram provided in the supplementary materials.
\end{quote}

Thank you very much for this suggestion. We plot 

\begin{quote}
How to use Wav2Lip to calculate $L_{sync}$?
\end{quote}

To calculate $L_{sync}$, following Wav2Lip, we first extract the video embedding $v$ and the speech embedding $s$ from the talking-head video and its corresponding speech. Next, we compute the cosine similarity between $v$ and $s$, which indicates the probability that the input audio-video pair is in sync. We then calculate $L_{sync}$ as the negative log-likelihood of this cosine similarity: $L_{sync} = -\textnormal{log} \frac{v \cdot s} {max(\lVert v \lVert \cdot \lVert s \lVert, \epsilon)}$, and minimize $L_{sync}$ during training. We will clarify this carefully.

\begin{quote}
In Section 4.1, how is the Emo-Acc metric calculated? Emotion category or intensity?
\end{quote}

The emotion accuracy metric is calculated based on emotion category. Specifically, we fine-tune an emotion recognition network, Emotion-Fan \cite{23}, using the training set of MEAD, following \cite{10}. This fine-tuned network is then used to predict the emotions of the generated talking-head videos.

\begin{quote}
Since the intensity is represented by the latent norm, how to classify them into slightly happy and extremely happy, which were mentioned in subsection 4.3.4. Is there a classification criteria?
\end{quote}

A:

\begin{quote}
How to evaluate the performance of the audio-to-intensity predictor?
\end{quote}

Thank you for the question. To evaluate the performance of the audio-to-intensity predictor, we measure the mean squared error (MSE) between the ground-truth emotion intensity and the intensity inferred by the predictor from the audio input. We split the Voxceleb2 dataset into a training set and a validation set. The MSE for the training set is 0.008, and for the validation set, it is 0.049, which corresponds to deviations of 1.4\% and 10.7\% from the ground-truth intensity, respectively. We will include these results.

\section*{Response to Reviewer NmsN}
\textbf{r/c - s/p/contribution}

\textbf{5/3 - 3/3/2}

We thank the reviewer for the valuable feedback. We address the major questions and concerns below.

\begin{quote}
From generation perspective, balancing emotion with lip movements is necessary, as the expression of certain emotions can affect the shape of the mouth. Using loss functions for joint constraints carries the risk of being difficult to balance. It is recommended to include ablation experiments on the selection of loss function coefficients.
\end{quote}

A: Thank you for the suggestion. In the main experiment, we set the lip-sync loss coefficient $\lambda_{sync}$ to be 10 and the expression regression loss coefficient $\lambda_{exp}$ to be 100. Additionally, we experiment with different coefficients as suggested. We observe a trade-off between emotion accuracy and lip-sync performance. As noted by the reviewer, the expression of certain emotions can affect the shape of the mouth, leading to this performance trade-off. We will include these results.

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
$\lambda_{sync}$ & 5 & 10 & 20 & 30 \\
\hline
SyncNet & 8.09 & 8.31 & 8.40 & 8.52 \\
Emo-Acc & 83.76 & 83.55 & 77.97 & 76.35 \\
\hline
\end{tabular}
\caption{Performance trade-offs with different loss coefficients.}
\end{table}

\begin{quote}
In the related work section, the used generator should be introduced in detail.
\end{quote}

A: Thank you for the suggestion. The generator used in our method is primarily derived from \cite{37}. It takes a set of 3D expression keypoints and the reference image as inputs to synthesize video frames. Specifically, the keypoints are first used to estimate warping flows, which are then applied to the features of the reference image to obtain warped features. These warped features are then inputted to a series of 2D residual blocks and upsampling layers to generate the final image. We will include these details in the related work section.

\begin{quote}
The paper seems to disregard the emotional signals contained in the audio. Would the emotional information in text conflict with the emotional information contained in the audio?
\end{quote}

A:

\begin{quote}
Regarding the reproducibility of the paper's methodology, is the talking head generator (Figure 1. Generator) used by this paper an open-source framework?
\end{quote}

Yes, our talking-head generator is primarily based on the one proposed in \cite{37}, which is an open-source framework. We will also publish the code for reproducibility.

\begin{quote}
Could you provide some analysis on the relationship between audio spectrograms and the predicted intensity of emotions?
\end{quote}

Thank you for the suggestion. We plot the relationship between audio spectrograms and the predicted emotion intensity as suggested (Figure 1 in the attached PDF). We observe that the predicted emotion intensity aligns well with the fluctuation in the audio spectrograms overall. For example, an increase in emotional intensity often corresponds to a noticeable change in energy levels within the audio spectrograms. This suggests that the speaking tone often reflects intensity fluctuations, and our model effectively captures these fluctuations based on audio inputs.

\section*{Response to Reviewer JHrF}

\textbf{r/c - s/p/contribution}

\textbf{6/4 - 3/3/2}

\begin{quote}
The chosen definition for "emotion intensity" does not seem to be validated in any way. It would have been preferable to draw on existing literature and definitions to define emotional intensity, and it would be important to validate this rating (e.g., by user study).
\end{quote}

Thank you for the suggestion.

\begin{quote}
Similarly, it is not clear to me that "emotion agnostic intensity" is a meaningful concept, and it would need to be validated specifically, for example, by testing large facial movements with no emotional content.
\end{quote}

A:

\begin{quote}
The method seems to perform very well and compares favourably to the chosen baselines, but it is not fully clear to me why this should be the case. I would have expected the emotional accuracy to improve, but why should the FID or the PSNR? In other words: why should the inclusion of the emotional intensity signal lead to the generation of more realistic images?
\end{quote}

A:

\begin{quote}
It would be interesting to break down the performance analysis per emotion (and per intensity). One would expect that some emotional expressions work better than others? Similarly, are there some faces from the dataset that lead to better/poorer performance?
\end{quote}

A:

\begin{quote}
The article does not really address the limitations of the method (section 5 only brushes on the notion of limitations, without substantial discussion). It is well established that AI applied on faces can lead to significant bias, due to poor representations on minorities.
\end{quote}

A:

\begin{quote}
Similarly, emotional expression varies depending on cultural background, and this is not really addressed.
\end{quote}

A:

